Exploiting Stability-Plasticity Asymmetry in Pretrained Detectors for Incremental Object Detection

Pretrained model-based incremental object detection (PTMIOD) leverages the rich detection priors of pretrained detectors to learn new categories incrementally while preserving detection ability on previously learned ones. Existing methods mainly exploit pretrained detectors as a whole, without explicitly distinguishing which components should remain stable and which require plastic adaptation. In this paper, we revisit PTMIOD from a component-wise stability-plasticity perspective. Our analysis of pretrained DETR-based detectors reveals a clear asymmetry: localization heads preserve transferable geometric priors across tasks, whereas classification-related representations require greater plasticity to handle new categories, especially in cross-domain scenarios where downstream data deviate from the pretraining domain. Based on this finding, we propose a selective adaptation and retention framework that freezes explicit localization heads to preserve localization stability, while adapting transformer representations with parameter-efficient fine-tuning and updating classification heads for classification-oriented plasticity. To alleviate classification-side forgetting, we pioneer the use of pseudo-feature replay in PTMIOD and design Quality-aware Gaussian Feature Replay, which estimates reliable class-wise feature distributions from high-quality matched object features and replays sampled pseudo features to maintain old-class decision boundaries. Since continual adaptation can shift the feature space and undermine replayed distributions, we further develop Two-stage Consistent Distillation to align teacher and student representations at both proposal generation and refinement stages.Extensive experiments on COCO, VOC, and TT100K show that our method achieves state-of-the-art performance, demonstrating a favorable balance between old-class retention and new-class adaptation.

==> tables/table_inference.tex <==
\begin{table}[t]
\centering
\caption{Comparison of parameter scale and efficiency. ``Total'' denotes deployment size. ``Trainable'' refers to updated parameters during initial ($t=1$) and incremental ($t>1$) steps. Latency is measured with batch size 1 on a GeForce RTX 3090 GPU.}
\label{tab:efficiency_comparison}
\begin{tabular}{l|cc}
\toprule
\textbf{Metric} & \textbf{MD-DETR}  & \textbf{Ours} \\
\midrule
Total (M) & 428.27 & \textbf{219.39} \\
Trainable ($t=1$) (M) & 208.79 & \textbf{0.37} \\
Trainable ($t>1$) (M) & 208.79 & \textbf{0.04} \\
Inference Latency (ms) & 292 & \textbf{193} \\
\bottomrule
\end{tabular}%
\end{table}

==> tables/table_loc_ablation.tex <==
\begin{table}[htbp]
\centering
\small % 直接用 small 控制自然字号，而不是强行缩放
\caption{Comparison of different training strategies for the Localization Head (LOC) under the 15-1 setting. ``Base-FT'' denotes fine-tuning only on the initial task, ``Cont-FT'' involves continuous fine-tuning across all tasks, and ``Frozen'' (Ours) indicates keeping the head completely fixed. Best results are highlighted in \textbf{bold}.}
\label{tab:loc_ablation}

% 稍微增加一点列间距，让数据呼吸
\setlength{\tabcolsep}{8pt}

% 去掉所有的竖线 |
\begin{tabular}{l ccc ccc}
\toprule
\multirow{2}{*}{\textbf{Strategy}} & \multicolumn{3}{c}{\textbf{VOC}} & \multicolumn{3}{c}{\textbf{TT100K}} \\ 
% 使用带有左右缩进(lr)的 cmidrule，代替丑陋的 \cline，视觉上更高级
\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
 & \textbf{1-15} & \textbf{16-20} & \textbf{1-20} & \textbf{1-15} & \textbf{16-20} & \textbf{1-20} \\ 
\midrule
Base-FT & 93.5 & 88.2 & 92.2 & 79.0 & 55.8 & 73.2 \\
Cont-FT & 93.6 & 87.9 & 92.2 & 77.7 & \textbf{56.3} & 72.4 \\
\textbf{Frozen} & \textbf{94.0} & \textbf{89.1} & \textbf{92.7} & \textbf{79.8} & 53.7 & \textbf{73.3} \\ 
\bottomrule
\end{tabular}
\end{table}

==> tables/table_loc_dis.tex <==
\begin{table}[t]
\centering
\caption{Component ablations under the 15--5 setting.}
\label{tab:ablation_component}
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{0.95}
\footnotesize
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Variant} & \multicolumn{3}{c}{VOC} & \multicolumn{3}{c}{TT100K} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& 1--15 & 16--20 & 1--20 & 1--15 & 16--20 & 1--20 \\
\midrule
\multicolumn{7}{l}{\textit{Distillation strategy}} \\
No KD       & 92.1 & 91.0 & 91.8 & 26.9 & 68.9 & 37.4 \\
Standard KD & --   & --   & --   & 36.4 & 51.0 & 40.1 \\
TFD         & 94.1 & 90.1 & 93.1 & 84.7 & 65.3 & 79.9 \\
\midrule
\multicolumn{7}{l}{\textit{Localization-head optimization}} \\
Tune loc. head   & --   & --   & --   & --   & --   & --   \\
Freeze loc. head & 94.1 & 90.1 & 93.1 & 84.7 & 65.3 & 79.9 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/table_params.tex <==
\begin{comment}
\begin{table}[h]
\centering
\caption{Parameter efficiency comparison of different methods. 'Backbone params' refers to the total number of parameters, while 'PEFT params' refers to the number of trainable parameters for each incremental task.}
\label{tab:param_efficiency}
\begin{tabular}{lcc}
\toprule
\textbf{Method} & \textbf{Backbone params} & \textbf{PEFT params} \\
\midrule
Faster ILOD & 32.8M & 32.8M \\
MMA & 32.8M & 32.8M \\
ABR & 32.8M & 32.8M \\
CL-DETR & 39.8M & 39.8M \\
\midrule % 使用midrule来分隔不同类型的模型
MD-DETR & 64.9M & 30.0M \\
\textbf{Ours} & \textbf{220.0M} & \textbf{0.04M} \\
\bottomrule
\end{tabular}
\end{table}
\end{comment}

\begin{table}[t]
\centering
\caption{Impact of different LoRA ranks ($r$) on mAP@50 for the VOC and TT100K datasets under the 15-5 setting.}
\label{tab:lora_rank}
\begin{tabular}{cccc}
\toprule
\textbf{Dataset} & \textbf{32} & \textbf{48} & \textbf{64} \\
\midrule
VOC & 93.3 & 93.1 & \textbf{93.4} \\
TT100K & 73.3 & \textbf{75.1} & 73.9 \\
\bottomrule
\end{tabular}
\end{table}

\begin{comment}
\begin{table}[t]
\centering
\caption{Parameter efficiency comparison.}
\label{tab:param_efficiency}
\begin{tabular}{lcc}
\toprule
\textbf{Method} & \textbf{Backbone params} & \textbf{PEFT params} \\
\midrule
Faster ILOD & 32.8M & - \\
MMA & 32.8M & - \\
ABR & 32.8M & - \\
CL-DETR & 39.8M & - \\
\midrule % 使用midrule来分隔不同类型的模型
MD-DETR & 64.9M & 30.0M \\
\textbf{Ours} & \textbf{220.0M} & \textbf{0.04M} \\
\bottomrule
\end{tabular}
\end{table}
\end{comment}


==> tables/table_storage.tex <==
\begin{table}[t]
\centering
\small
\caption{Parameter and efficiency comparison. Trainable parameters are reported for task \(t=1\), and storage is computed from task-specific trainable parameters under FP32 precision. Lower is better.}
\label{tab:efficiency_comparison}
\setlength{\tabcolsep}{3.8pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{l|ccc}
\toprule
\textbf{Method} & \textbf{Trainable (M)} & \textbf{Storage (MB)} & \textbf{Latency (ms)} \\
\midrule
MD-DETR~\cite{bhatt2024preventing} & $208+0.46\times t$ & 0 & 292 \\
P$^2$IOD                           & 5.98   & $20\times t$  & 282 \\
\rowcolor{gray!8}
Ours                               & 0.53 & $1.13\times n$ & 193 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/table_tt_voc_mul_tasks.tex <==
\begin{table*}[t]
\caption{mAP@50 results of VOC and TT100K on multi-increment setting. The best result in each column is \textbf{bolded}, and the second-best result is \underline{underlined}. Methods with $^\dagger$ means results of VOC from our re-implementation.}
\label{tab:mi_pt}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc||ccc|ccc} 
\hline
\multicolumn{1}{l|}{\textbf{Dataset}} & \multicolumn{6}{c||}{\textbf{VOC}} & \multicolumn{6}{c}{\textbf{TT100K}} \\ 
\hline
\textbf{Setting} & \multicolumn{3}{c|}{\textbf{10-5 (3 Tasks)}} & \multicolumn{3}{c||}{\textbf{15-1 (6 Tasks)}} & \multicolumn{3}{c|}{\textbf{10-5 (3 Tasks)}} & \multicolumn{3}{c}{\textbf{15-1 (6 Tasks)}} \\ 
\hline
\textbf{Method} & \textbf{1-10} & \textbf{11-20} & \cellcolor{gray!30} \textbf{1-20} & \textbf{1-15} & \textbf{16-20} & \cellcolor{gray!30} \textbf{1-20} & \textbf{1-10} & \textbf{11-20} & \cellcolor{gray!30} \textbf{1-20} & \textbf{1-15} & \textbf{16-20} & \cellcolor{gray!30} \textbf{1-20} \\ 
\hline
Faster ILOD & 68.3 & 57.9 & \cellcolor{gray!30} 63.1 & 66.9 & 44.5 & \cellcolor{gray!30} 61.3 & 45.6 & 19.5 & \cellcolor{gray!30} 32.6 & \underline{47.2} & 24.2 & \cellcolor{gray!30} \underline{41.4} \\
MMA & 67.4 & 60.5 & \cellcolor{gray!30} 64.0 & 67.2 & 47.8 & \cellcolor{gray!30} 62.3 & 50.8 & 26.3 & \cellcolor{gray!30} 38.6 & 43.5 & 29.0 & \cellcolor{gray!30} 39.9 \\
ABR & 68.7 & 67.1 & \cellcolor{gray!30} 67.9 & \underline{68.7} & \underline{56.7} & \cellcolor{gray!30} \underline{65.7} & \underline{52.5} & \underline{33.8} & \cellcolor{gray!30} \underline{43.1} & 43.1 & \underline{35.4} & \cellcolor{gray!30} 41.0 \\
CL-DETR$^\dagger$ & 15.0 & 26.1 & \cellcolor{gray!30} 20.6 & 45.3 & 10.1 & \cellcolor{gray!30} 36.5 & 49.8 & 28.0 & \cellcolor{gray!30} 38.9 & 30.8 & 9.4 & \cellcolor{gray!30} 25.4 \\ 
MD-DETR$^\dagger$ & \underline{80.1} & \underline{87.5} & \cellcolor{gray!30} \underline{83.8} & 38.0 & 1.1 & \cellcolor{gray!30} 28.8 & 0.3 & 18.7 & \cellcolor{gray!30} 9.3 & 0.1 & 2.3 & \cellcolor{gray!30} 0.6 \\
\hline
\hline
Ours & \textbf{94.3} & \textbf{90.0} & \cellcolor{gray!30} \textbf{92.2} & \textbf{94.0} & \textbf{89.1} & \cellcolor{gray!30} \textbf{92.7} & \textbf{69.3} & \textbf{47.3} & \cellcolor{gray!30} \textbf{58.3} & \textbf{79.8} & \textbf{53.7} & \cellcolor{gray!30} \textbf{73.3} \\ 
\hline
\end{tabular}
}
\end{table*}

==> tables/table_tt_voc_two_tasks.tex <==
\begin{table*}[t]
\caption{mAP@50 results of VOC and TT100K on single-increment setting. The best result in each column is \textbf{bolded}, and the second-best result is \underline{underlined}. Methods with $^\dagger$ means results of VOC from our re-implementation. }
\label{tab:si_pt}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc||ccc|ccc} 
\hline
\multicolumn{1}{l|}{\textbf{Dataset}} & \multicolumn{6}{c||}{\textbf{VOC}} & \multicolumn{6}{c}{\textbf{TT100K}} \\ 
\hline
\textbf{Setting} & \multicolumn{3}{c|}{\textbf{10-10}} & \multicolumn{3}{c||}{\textbf{15-5}} & \multicolumn{3}{c|}{\textbf{10-10}} & \multicolumn{3}{c}{\textbf{15-5}} \\ 
\hline
\textbf{Method} & \textbf{1-10} & \textbf{11-20} & \cellcolor{gray!30} \textbf{1-20} & \textbf{1-15} & \textbf{16-20} & \cellcolor{gray!30} \textbf{1-20} & \textbf{1-10} & \textbf{11-20} & \cellcolor{gray!30} \textbf{1-20} & \textbf{1-15} & \textbf{16-20} & \cellcolor{gray!30} \textbf{1-20} \\ 
\hline
Faster ILOD & 70.3 & 53.0 & \cellcolor{gray!30} 61.7 & 73.1 & 57.3 & \cellcolor{gray!30} 69.2 & 49.1 & 21.2 & \cellcolor{gray!30} 35.2 & 46.7 & 27.3 & \cellcolor{gray!30} 41.9 \\
MMA & 69.8 & 63.9 & \cellcolor{gray!30} 66.8 & 72.7 & 60.6 & \cellcolor{gray!30} 69.7 & 48.1 & 28.0 & \cellcolor{gray!30} 38.1 & 44.4 & 35.4 & \cellcolor{gray!30} 42.2 \\
ABR & 71.2 & 72.8 & \cellcolor{gray!30} 72.0 & 73.0 & 65.1 & \cellcolor{gray!30} 71.0 & 55.0 & \underline{39.3} & \cellcolor{gray!30} \underline{47.2} & \underline{47.3} & 39.0 & \cellcolor{gray!30} \underline{45.6} \\
CL-DETR$^\dagger$ & 45.2 & 56.0 & \cellcolor{gray!30} 50.6 & 52.1 & 38.2 & \cellcolor{gray!30} 48.6 & \underline{52.1} & 37.5 & \cellcolor{gray!30} 44.8 & 36.8 & \underline{43.9} & \cellcolor{gray!30} 38.6 \\ 
MD-DETR$^\dagger$ & \underline{81.8} & \underline{87.3} & \cellcolor{gray!30} \underline{84.6} & \underline{86.1} & \underline{84.7} & \cellcolor{gray!30} \underline{85.8} & 0.1 & 37.1 & \cellcolor{gray!30} 18.6 & 0.5 & 39.1 & \cellcolor{gray!30} 9.8 \\
\hline
\hline
Ours & \textbf{94.4} & \textbf{90.7} & \cellcolor{gray!30} \textbf{92.5} & \textbf{94.7} & \textbf{88.1} & \cellcolor{gray!30} \textbf{93.1} & \textbf{77.8} & \textbf{51.5} & \cellcolor{gray!30} \textbf{64.6} & \textbf{78.8} & \textbf{63.9} & \cellcolor{gray!30} \textbf{75.1} \\ 
\hline
\end{tabular}
}
\end{table*}
